Learning to Incentivize Information Acquisition: Proper Scoring Rules Meet Principal-Agent Model

We study the incentivized information acquisition problem, where a principal hires an agent to gather information on her behalf. Such a problem is modeled as a Stackelberg game between the principal and the agent, where the principal announces a scoring rule that specifies the payment, and then the agent then chooses an effort level that maximizes her own profit and reports the information. We study the online setting of such a problem from the principal's perspective, i.e., designing the optimal scoring rule by repeatedly interacting with the strategic agent. We design a provably sample efficient algorithm that tailors the UCB algorithm (Auer et al., 2002) to our model, which achieves a sublinear $T^{2/3}$-regret after $T$ iterations. Our algorithm features a delicate estimation procedure for the optimal profit of the principal, and a conservative correction scheme that ensures the desired agent's actions are incentivized. Furthermore, a key feature of our regret bound is that it is independent of the number of states of the environment.

==> macro.tex <==
\RequirePackage{bm} 

\newtheorem{theorem}{Theorem} 
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}[theorem]{Example}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{note}[theorem]{Note}
\newtheorem{asum}[theorem]{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheoremstyle{nonindented}{1ex}{1ex}{}{}{\bfseries}{.}{.5em}{}
\newtheoremstyle{indented}{1ex}{1ex}{\itshape\addtolength{\leftskip}{0.6cm}\addtolength{\rightskip}{0.6cm}}{}{\bfseries}{.}{.5em}{}
\theoremstyle{nonindented}
%\newtheorem{domain}{Game Domain}
\theoremstyle{indented}
\newtheorem{ind_definition}[theorem]{Definition}
\newtheorem{ind_lemma}[theorem]{Lemma}
%\newtheorem{question}{Question}[section]
%\newtheorem*{direction*}{Research Direction}
%\newtheorem*{conjecture*}{Conjecture}
\theoremstyle{plain}



\newenvironment{proofof}[1]{\begin{proof}[Proof of #1]}{\end{proof}}
\newenvironment{proofsketch}{\begin{proof}[Proof Sketch]}{\end{proof}}
\newenvironment{proofsketchof}[1]{\begin{proof}[Proof Sketch of #1]}{\end{proof}}

\newenvironment{alg}{\begin{algorithm}\begin{onehalfspace}\begin{algorithmic}[1]}{\end{algorithmic}\end{onehalfspace}\end{algorithm}} 

\newcommand{\bv}{\mathbf}
\newcommand{\mult}{\times}
\newcommand{\cross}{\times}
\newcommand{\by}{\times}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\card}[1]{\left| #1 \right|}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}
\newcommand{\bigunion}{\bigcup}
\newcommand{\bigintersect}{\bigcap}
\newcommand{\sm}{\setminus}
\newcommand{\floor}[1]{\lfloor {#1} \rfloor}
\newcommand{\ceil}[1]{\lceil {#1} \rceil}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}
\newcommand{\iid}{i.i.d.\ }
\newcommand{\bvec}[1]{\boldsymbol{ #1 }}

\newcommand{\lt}{\left}
\newcommand{\rt}{\right}

%%%%% Norms

\newcommand{\norm}[1]{||#1||}
\newcommand{\bignorm}[1]{\bigg|\bigg|#1\bigg|\bigg|}
\newcommand{\opnorm}[2]{| \! | \! | #1 | \! | \! |_{{#2}}}


\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}

\DeclareMathOperator{\UCB}{UCB}
\DeclareMathOperator{\Reg}{Reg}
\DeclareMathOperator{\Vol}{Vol}

%Operators: These operators are such that a subscript appears below
%in \[ \] math mode, and to the bottom right in regular $ $ math mode

%regular version
\def\pr{\qopname\relax n{Pr}}
\def\ex{\qopname\relax n{E}}
\def\min{\qopname\relax n{min}}
\def\max{\qopname\relax n{max}}
\def\maxs{\qopname\relax n{max2}}
\def\argmin{\qopname\relax n{argmin}}
\def\argmax{\qopname\relax n{argmax}}
\def\avg{\qopname\relax n{avg}}


%bold version
\def\Pr{\qopname\relax n{\mathbf{Pr}}}
\def\Ex{\qopname\relax n{\mathbf{E}}}
\def\supp{\qopname\relax n{\mathbf{supp}}}
\def\Min{\qopname\relax n{\mathbf{min}}}
\def\Max{\qopname\relax n{\mathbf{max}}}
\def\Argmin{\qopname\relax n{\mathbf{argmin}}}
\def\Argmax{\qopname\relax n{\mathbf{argmax}}}
\def\Avg{\qopname\relax n{\mathbf{avg}}}
\def\vol{\qopname\relax n{\mathbf{vol}}}
\def\aff{\qopname\relax n{\mathbf{aff}}}
\def\conv{\qopname\relax n{\mathbf{convexhull}}}
\def\hull{\qopname\relax n{\mathbf{hull}}}

\newcommand{\expect}[2][]{\ex_{#1} [#2]}

% \newcommand{\RR}{\mathbb{R}}
\newcommand{\RRp}{\RR_+}
\newcommand{\RRpp}{\RR_{++}}
% \newcommand{\NN}{\mathbb{N}}
% \newcommand{\ZZ}{\mathbb{Z}}
% \newcommand{\QQ}{\mathbb{Q}}
% \newcommand{\PP}{\mathbb{P}}

% \def\A{\mathcal{A}}
% \def\B{\mathcal{B}}
% \def\C{\mathcal{C}}
% \def\D{\mathcal{D}}
% \def\E{\mathcal{E}}
% \def\F{\mathcal{F}}
% \def\G{\mathcal{G}}
% \def\H{\mathcal{H}}
% \def\I{\mathcal{I}}
% \def\J{\mathcal{J}}
% \def\L{\mathcal{L}}
% \def\M{\mathcal{M}}
% \def\P{\mathcal{P}}
% \def\R{\mathcal{R}}
% \def\S{\mathcal{S}}
% \def\O{\mathcal{O}}
% \def\T{\mathcal{T}}
% \def\V{\mathcal{V}}
% \def\X{\mathcal{X}}
% \def\Y{\mathcal{Y}}

%----- bold fonts -----%

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
% \newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
% \newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%----- blackboard bold fonts-----%

\newcommand{\CC}{\mathbb{C}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\B}{{\mathbb B}}

%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bomega}{\bm{\omega}}
\newcommand{\bdelta}{\bm{\delta}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}


\def\eps{\epsilon}
\def\sse{\subseteq}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\Bmat}[1]{\begin{Bmatrix} #1 \end{Bmatrix}}
\newcommand{\vmat}[1]{\begin{vmatrix} #1 \end{vmatrix}}
\newcommand{\Vmat}[1]{\begin{Vmatrix} #1 \end{Vmatrix}}
\newcommand{\mat}[1]{\pmat{#1}}
\newcommand{\grad}{\bigtriangledown}
\newcommand{\one}{{\bf 1}}
\newcommand{\zero}{{\bf 0}}


\newcommand{\hl}[1]{{\bf \color{red}#1}}
% \newcommand{\todo}[1]{{\hl{To do: #1}}}
\newcommand{\todof}[1]{{\hl{ (Todo\footnote{\hl{\bf  To do: #1}})}}  }
\newcommand{\noi}{\noindent}
\newcommand{\prob}[1]{\vspace{.2in} \noindent {\bf Problem #1.}\\}
\newcommand{\subprob}[1]{ \vspace{.2in} \noindent {\bf #1.}\\}


%Plain eps or pdf figure. Use IPE to embed tex in it.
\newcommand{\fig}[2][1.0]{
  \begin{center}
    \includegraphics[scale=#1]{#2}
  \end{center}}
%Combined PS/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined ps/latex" option
\newcommand{\figpst}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pstex_t}}
  \end{center}}
%Combined PDF/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined pdf/latex" option
\newcommand{\figpdft}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pdf_t}}
  \end{center}}



%Algorithmic Environment stuff
\newcommand{\INPUT}{\item[\textbf{Input:}]}
\newcommand{\OUTPUT}{\item[\textbf{Output:}]}
\newcommand{\PARAMETER}{\item[\textbf{Parameter:}]}


%LP environment stuff
\newcommand{\mini}[1]{\mbox{minimize} & {#1} &\\}
\newcommand{\maxi}[1]{\mbox{maximize} & {#1 } & \\}
\newcommand{\maximin}[1]{\mbox{max min} & {#1 } & \\}
\newcommand{\find}[1]{\mbox{find} & {#1 } & \\}
\newcommand{\st}{\mbox{subject to} }
\newcommand{\con}[1]{&#1 & \\}
\newcommand{\qcon}[2]{&#1, & \mbox{for } #2.  \\}
\newenvironment{lp}{\begin{equation}  \begin{array}{lll}}{\end{array}\end{equation}}
\newenvironment{lp*}{\begin{equation*}  \begin{array}{lll}}{\end{array}\end{equation*}}



%% MISC





==> related-work-brief.tex <==
\subsection{Related Work}
The information elicitation problem and its implications for decision making have been one of the most popular areas in economics. The seminal work by \cite{savage1971elicitation} characterizes the truthful elicitation with the design of proper scoring rules. More recently, several work have studied the optimization problem of scoring rules for the principal's different objectives~\cite{CY-21,li2022optimization,10.1145/3490486.3538261, neyman2021binary}. Closer to our problem is the model studied by \citet{10.1145/3490486.3538261,oesterheld2020minimum}, as we both explore the connection between information acquisition and contract design. However, our model is strictly more general in that we assume the agent may have multi-level efforts, and the information state may be affected by the agent's action. In addition, we primarily focus on the learning aspects, when the principal has limited knowledge of the game parameters. 

More generally, our problem is related to a family of online learning problems under the principal-agent framework, which includes special cases such as security game, information design, auction design, contract design and etc. However, to our best knowledge, there is no previous work that considered any similar learning problem for our model of information acquisition. We also remark that, in many of these existing works, e.g.,~\citet{balcan2015commitment,guo2022no,castiglioni2020online,wu2022sequential}, the learner is assumed to have sufficient knowledge about the other strategic player(s), and her uncertainty is regarding the environment or her own utility. Assumptions of such kind can significantly simplify the problem into the standard online learning problems, once the learner can almost predict the best response of other player(s). Notably, our work does not make any of such assumption and the most challenging part of our learning algorithm design is indeed to ensure the desired agent response under uncertainty. 
We defer more discussions on the related work to \Cref{sec:related-work-full}.
